Learning Multimodal VAEs through Mutual Supervision

Multimodal VAEs seek to model the joint distribution over heterogeneous data (e.g.\ vision, language), whilst also capturing a shared representation across such modalities. Prior work has typically combined information from the modalities by reconciling idiosyncratic representations directly in the recognition model through explicit products, mixtures, or other such factorisations. Here we introduce a novel alternative, the MEME, that avoids such explicit combinations by repurposing semi-supervised VAEs to combine information between modalities implicitly through mutual supervision. This formulation naturally allows learning from partially-observed data where some modalities can be entirely missing -- something that most existing approaches either cannot handle, or do so to a limited extent. We demonstrate that MEME outperforms baselines on standard metrics across both partial and complete observation schemes on the MNIST-SVHN (image-image) and CUB (image-text) datasets. We also contrast the quality of the representations learnt by mutual supervision against standard approaches and observe interesting trends in its ability to capture relatedness between data.

==> 1introduction_v1.tex <==


\section{Introduction}
%
Machine learning practitioners are often faced with the task of reconciling relevant data from multiple heterogenic sources and types, for instance, images of similar abstract content, but very different concrete visualisations.
%
Alternatively, image or numerical data might come paired with textual descriptive information. 
%
Such data, consisting of related but heterogeneous types and sources are commonly referred to as \emph{multimodal}.
%
Learning representations in the context of multimodal data often aims at utilising commonalities to find mutual abstract concepts.


%Multimodal learning in generative models often aims at learning common abstract concept from multiple modalities.
%
Techniques incorporating the multimodal nature of the data have been shown to yield more generalisable representations~\citep{zhang2020multimodal, guo2019deep, yildirim2014from}, however, they are often exposed to the following problems:
%they often require paired data from all modalities to be available at train time to learn a joint probabilistic representation.
%
%There are two issues with this school of thinking: 1) \emph{data efficiency}, since constructing multimodal datasets with paired examples can require a large amount of annotated data from unimodal datasets, and 2) \emph{"artificial" joint posterior}, the posterior from each modality often needs some pre-determined mechanism to be fused together to form the joint posterior, either by factorising unimodal posterior using \gls{MoE}~\citep{Shi2019},  \gls{PoE}~\citep{Wu2018b} or by defining a joint encoder~\citep{JMVAE_suzuki_1611,JVAE_pu_2016}.
%Here, we highlight two shortcomings common to many current approaches: 
1) \emph{data efficiency}; since constructing multimodal data sets with paired examples can require a large amount of laborious data annotation from unimodal datasets, and 2) \emph{reconciling modality idiosyncratic distributions}, the distributions of individual modalities require some mechanism to be fused to form a joint probabilistic representation.
%
In practice, the latter can be achieved by treating the individual representations as experts, which can by subsequently combined by, e.g. linear \gls{MoE}~\citep{Shi2019} or logarithmic  \gls{PoE}~\citep{Wu2018b} pooling, or, alternatively by defining a joint  encoder~\citep{JMVAE_suzuki_1611,TELBO_vedantam_1705, tsai2018learning}.

{\color{blue}
A conceptual problem of the \gls{PoE} and \gls{MoE} approaches arises when individual experts have discordant views on the representations. To see this consider \cref{fig:abs}. \glspl{PoE} can be seen as choosing a \enquote{minimal common denominator} representation. For discordant views \gls{PoE} therefore could be forced to agree on representations that are not very pertinent to either modality. 
On the other hand, \glspl{MoE} might fuse both representations without ensuring universality of the common representation.  
}


Here, we introduce an alternative approach that we term \gls{MEME}, which does {\bfseries not} combine the individual experts.
%
Instead, we treat the individual experts as stand-alone representations, removing the need to reconcile the idiosyncrasies of the individual encoding distributions.
%
Critically, doing so allows the formulation of a principled approach to dealing with the case when the modalities are partially observed.

Problems arising from missing or partially observed data have seen increasing attention in last years---for example, the handling of missing labels has been discussed under the umbrella term \enquote{semi-supervised} \gls{VAE}~\citep[see e.g.][]{kingma2014semi,joy2021capturing, maaloe2017semi, siddharth2017learning, ilse2019diva}.
%
This paradigm can be viewed as the special case of multimodal VAEs, where in this case, the \emph{labels} represent a modality.
%
In this work, we see how the insights of~\cite{joy2021capturing} can be re-purposed to learn multi-modal VAEs when the data is partially observed.

Specifically, rather than combining individual experts to obtain a joint representation, e.g. see Left and Middle of \cref{fig:abs}.
%
We instead regularize the individual experts to minimize a divergence between themselves, thus placing the embeddings for each modality in similar regions of the latent space, \cref{fig:abs} Right.
%
Thus, when observing only one modality, the latent representation remains the same.
%
Unlike for the PoE, which will change the green distribution if we only observe the blue modality, creating a miss-match between the representations in fully observed and partially observed case.
 
As we will show, our approach provides superior performance in the partially observed training paradigm.
%
We highlight the advantages of our approach below:
%
\begin{itemize}
    \item By merit of the semi-supervised construction, our model deals with partially observed inputs during training without having to sub-sample modalities or architectural components;
    \item We develop a more principled approach for the interactions between two modalities through mutual regularization. As a result, we no longer need to define a joint posterior or any artificial mechanism to manufacture the interactions of representations between modalities;
    \item Our objective naturally contains a measure of ``relatedness'', which can be used to identify similar samples and offer insights on the learning of the model.
\end{itemize}





% Several data modalities in the wild often represent the same underlying abstract concept, for instance a natural language caption and image of the same object/scene or two pictures of the same digit.
% %
% Provided with these modalities, algorithms should be able to learn representations that faithfully capture the information from both data sources.
% %
% %In fact, there is evidence to suggest that we as humans undergo a similar learning process~\cite{quiorga, stein}. 
% %
% Learning joint representations enables the ability to perform cross-generation between modalities by treating the representation as intermediary layers.
% %
% Furthermore, multiple modalities should give rise to more robust feature representations.

% A suitable framework for learning representations is the VAE.
% %
% Existing work on multi-modal learning in VAEs typically combines the multiple modalities in the inference modal.
% %
% Doing so requires that the individual approximate posteriors for each modality are joined through either a Product of Experts (PoE)~\cite{Wu2018b} or a Mixture of Experts (MoE)~\cite{Shi2019}, with their associated disadvantages.
% %
% Using a PoE~\cite{Wu2018b} requires that the data needs to sub-sampled during training to ensure the encoder learns anything meaningful.
% %
% Furthermore, the PoE is not particularly well suited to multi-modal learning~\cite{Shi2019}, as the standard-deviation of each expert will drastically affect the resulting posterior, which poses a significant problem if they are miss-calibrated, see \cref{fig:abs} (Left).
% %
% Whilst in~\cite{Shi2019}, the formulation of the approximate posterior as a mixture of the experts places the hard constrain that data for each modality is always present, completely removing the possibility of weakly-supervised learning.
% %
% Moreover, the weighting of each modality has to be heuristically chosen, which if chosen incorrectly can lead to poor posterior distributions, see \cref{fig:abs} (Middle).
% %
% We propose a novel method that achieves the desired objectives of multi-modal learning in VAEs without inducing the penalty of the above deficiencies.

\begin{figure}
	\begin{tabular}{ccc}
		\includegraphics[width=0.3\linewidth]{media/poe.png}&
		\includegraphics[width=0.3\linewidth]{media/moe.png}&
		\includegraphics[width=0.3\linewidth]{media/ours.png}
	\end{tabular}
	\caption{Graphical interpretation of the PoE~\citep{Wu2018b} (left), MoE~\citep{Shi2019} (middle) and our approach (right). Here we can see that the PoE completely disregards the contribution by expert two; the requirement for all modalities to be present in MoE; and that ours will construct distributions that match.}
	\label{fig:abs}
\end{figure}

% Obtaining data pairs is expensive and energy intensive.
% %
% Naturally, we want to learn representations in situations where we might not always have matching data pairs.
% %
% This weakly-supervised case is amenable in ~\cite{Wu2018b}, but not possible in ~\cite{Shi2019}.
% %
% Furthermore, a joint representation should provide some notion of \emph{relatedness} between modalities, i.e. how similar is a data point $\x_j$ to $\x_i$.
% %
% Due to the construction of the PoE and the MoE, it is not clear how one would extract this metric.
% %
% These two objectives are the aim of this work, namely:

% \begin{itemize}
% 	\item principally deal with the weakly-supervised case without introducing issues from the PoE.
% 	\item how to construct a measure of relatedness between data points from different modalities.
% \end{itemize}


% We propose a method that avoids combining the modalities in the inference modal.
% %
% Instead, we seek to obtain a joint representation by taking a top-down/bottom-up approach.
% %
% Where we combine the bottom-up information from one modality with the top-down information from another.
% %
% Specifically, we seek to regularize the approximate posterior for modality $S$ with a conditional prior from $T$.
% %
% We introduce our graphical model in \cref{fig:model}, where it can be seen that the bottom-up inference model from $\bs$ is regularized by the top-down generative model from $\bt$.
% %
% This provides a flexible way to obtain joint representations through regularization, removing the need to explicitly join the modalities like in~\cite{Wu2018b, Shi2019}.
%
% We summarise the features of our model and contrast them with~\cite{Wu2018b, Shi2019} in \cref{tab:comparison}. We also conceptually highlight our approach in~\cref{fig:abs}.
% %
% Specifically our contributions are as follows:
% %
% \begin{itemize}
% 	\item Introduce multi-modal VAEs through a bottom-up/top-down approach, alleviating the need to combine experts in the inference model.
% 	\item Formulate multi-model VAEs when we have incomplete data.
% 	\item Highlight how our modal can deal with relatedness.
% 	\item Demonstrate that the bottom-up/top-down approach is superior to the combination of experts approach.
% \end{itemize}

%
% \begin{table}[h]
% 	\centering
% 	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
% 	\caption{Comparison of Models.}
% 	{\small
% 		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\s}}
% 			\toprule
% 			& MVAE~\citep{Wu2018b} & MMVAE~\citep{Shi2019} & Ours\\
% 			\midrule
% 			Requires sub-sampling during training & \xmark & \cmark & \cmark \\
% 			Can perform semi-supervised learning & \cmark & \xmark & \cmark \\
% 			Can extract relatedness & \xmark & \xmark & \cmark \\
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\label{tab:comparison}
% \end{table}



==> 1introduction_v2.tex <==
\section{Introduction}
%
Multimodal data refers to data that contains related but heterogeneous types and sources, for instance realistic photos and sketches that depict identical abstract concept, or caption and image from the same scene.
%
Learning representations in the context of multimodal data often aims at utilising commonalities to find mutual abstract concepts.

Multimodal \glspl{VAE} have been shown to yield more generalisable representations~\citep{zhang2020multimodal, guo2019deep, Shi2019}.
%
However, these models often require paired data from both modalities to be available at train time.
%
Since constructing multimodal datasets with paired examples can require a large amount of annotated data from unimodal datasets, training these models can be expensive.


%
% This regime is explosed to the following two problems: 1) \emph{data efficiency}, since constructing multimodal datasets with paired examples can require a large amount of annotated data from unimodal datasets, and
%
% 2) \emph{artificial reconciliation of idiosyncratic distribution}, the representation distribution of each modality often needs some pre-determined mechanism to be aligned/fused to form a joint distribution, either by factorising unimodal posterior using \gls{MoE}~\citep{Shi2019},  \gls{PoE}~\citep{Wu2018b} or by defining a joint encoder~\citep{JMVAE_suzuki_1611,JVAE_pu_2016}.

Several work have attempted to address this issue.
%
\citet{Wu2018b}, \citet{gong21} and \citet{sutter2021generalized}, address the data efficiency issue by designing models that can learn from incomplete set of modalities during training.
%
However, all of these methods require additional components/steps to handle missing modalities at train time, and only \citet{gong21} empirically verified the model's performance under partially observed multimodal data.
%
Further, \citet{shi2021relating} proposed a contrastive \gls{ELBO} that learns a \enquote{relatedness} metric, which can then be used to identify paired data from unlabelled multimodal dataset to use for training.
%
However, their method make assumptions on the missingness mechanism \citep{little1987statistical} and is only effective when data are missing at random --- if data from only one modality is missing, no paired samples can be leveraged for further training.\todo{I'm not sure talking about relatedness fits in here}

Despite its challenges, missing inputs itself is not a novel concept --- in fact, missing labels has been widely discussed in the realm of semi-supervised VAE (see e.g.~\citet{ilse2019diva, kingma2014semi,joy2021capturing, maaloe2017semi, siddharth2017learning}.
%
In this work, we consider this paradigm as a special case for multimodal \glspl{VAE} by viewing \emph{labels} as a modality.
%
Under the semi-supervised VAE umbrella, we can now learn from partially-observed multimodal data without any additional components or training steps.
%
As we will show, our proposed model, \gls{MEME}\footnote{Chosen from multiple options by optimising across relevance (higher), length (lower), tediousness (lower) and flippancy (moderate)}, achieves strong empirical results when large amount of data from one or either modalities are missing.
%
More specifically, our approach has the following advantages:
%
\begin{itemize}
    \item Our model learns from partially observed multimodal data effectively, without additional components/training step or assumption on missingness mechanism (i.e. missing data can be in either modality or in one modality only);
    \item By adopting a semi-supervised framework, we develop a more principled approach for the reconciliation between modality distributions and achieve better representation quality;
    \item Our objective naturally contains a measure of ``relatedness'', which can be used to identify more paired sample and offer insights on the learning of the model.
\end{itemize}


\todo{Jimmy: I believe the following can go into the problem formulation section}

{\color{blue}
A conceptual problem of the \gls{PoE} and \gls{MoE} approaches arises when individual experts have discordant views on the representations. To see this consider \cref{fig:abs}. \glspl{PoE} can be seen as choosing a \enquote{minimal common denominator} representation. For discordant views \gls{PoE} therefore could be forced to agree on representations that are not very pertinent to either modality.
On the other hand, \glspl{MoE} might fuse both representations without ensuring universality of the common representation.
}

Specifically, rather than combining individual experts to obtain a joint representation, e.g. see Left and Middle of \cref{fig:abs}.
%
We instead regularize the individual experts to minimize a divergence between themselves, thus placing the embeddings for each modality in similar regions of the latent space, \cref{fig:abs} Right.
%
Thus, when observing only one modality, the latent representation remains the same.
%
Unlike for the PoE, which will change the green distribution if we only observe the blue modality, creating a miss-match between the representations in fully observed and partially observed case.

As we will show, our approach provides superior performance in the partially observed training paradigm.
%
We highlight the advantages of our approach below:
.

\begin{figure}
	\begin{tabular}{ccc}
		\includegraphics[width=0.3\linewidth]{media/poe.png}&
		\includegraphics[width=0.3\linewidth]{media/moe.png}&
		\includegraphics[width=0.3\linewidth]{media/ours.png}
	\end{tabular}
	\caption{Graphical interpretation of the PoE~\citep{Wu2018b} (left), MoE~\citep{Shi2019} (middle) and our approach (right). Here we can see that the PoE completely disregards the contribution by expert two; the requirement for all modalities to be present in MoE; and that ours will construct distributions that match.}
	\label{fig:abs}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 1introduction_v3.tex <==
\section{Introduction}
%
Multimodal data refers to data that contains related but heterogeneous types and sources, for instance realistic photos and sketches that depict identical abstract concepts, or caption and image data from the same scene.
%
Learning representations in the context of multimodal data often aims at finding latent variables associated with such mutual abstract concepts.

Multimodal \glspl{VAE} have been shown to yield more generalisable representations~\citep{zhang2020multimodal, guo2019deep, Shi2019}.
%
However, past work on multimodal \glspl{VAE} often leverages some \emph{explicit} combinations between the modalities to learn either joint or aligned distributions between modalities.
%
This is done either through concatenating multimodal inputs \citep{JMVAE_suzuki_1611,TELBO_vedantam_1705, tsai2018learning}, latents \citep{gong21}, or factorising the joint distribution as \gls{PoE} \citep{Wu2018b} or \gls{MoE} \citep{Shi2019} of unimodal experts.
%
While these work have achieved interesting results, it's difficult to offer sufficient justification for the explicit mechanism chosen to fuse information from multiple modalities.
\todo{Jimmy: I hesitate with this sentence as it might be too strong a statement, consider replacing it by "justification are often required for the explicit mechanism used to fuse information from multiple modalities"}
%
In addition, the model often requires extra components/training steps to learn balanced representations.

Multimodal \glspl{VAE} are not unique in their pursuit to learn better probabilistic representations by combining information from multiple sources.
%
Conceptually closely related are semi-supervised \glspl{VAE} (see e.g. \citet{ilse2019diva, joy2021capturing, kingma2014semi, maaloe2017semi, siddharth2017learning}), where labels are used as an additional source of information to supervise the learning of the data.
%
In particular, data is considered in input-output pairs, where labels induce learning of features that are pertinent to the output. 
%
Drawing inspiration from this, we propose to re-purpose semi-supervised \glspl{VAE} for the learning of multimodal data, by recognizing that paired modalities offer additional information similar to label descriptions.
%
This allows us to combine information shared between modalities in an \emph{implicit} manner, where each modality supervises the learning of the other by leading the learned representations to be predictive of their respective pair.
%
Our proposed model \gls{MEME}\footnote{Chosen from multiple options by optimising across relevance (higher), length (lower), tediousness (lower) and flippancy (moderate)} has the following advantages:
%
\begin{itemize}
    \item \gls{MEME} can naturally learn from partially-observed multimodal data without additional components/training steps---in contrast to other existing approaches, such as \citet{Wu2018b, sutter2020multimodal, gong21};
    \item As we show in experiments, \gls{MEME} outperforms baselines on standard metrics where training is performed under both complete and partial data;
    \item Our objective naturally contains a measure of \enquote{relatedness}, which can be used to measure the extend to which samples are paired and thus offer insights on the learning of the model.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 2_5problemformulation.tex <==
\section{Problem Formulation}\label{sec:3}
%
\todo[inline]{Don't get into the architecture, talk about distinctions between other approaches, move this further up}
%
Previous approaches typically combine experts in the inference model~\citep{sutter2021generalized, Shi2019, Wu2018b}, which facilitates a way to combine information from both modalities.
%
Here we discuss whether this is appropriate for situations where the modalities are partially observed.

When comparing situations where one of the modalities is observed and when it is unobserved, it is natural to ask the question `what should happen to the latent code'?
%
Should it remain the same? Or should it differ?
%
Before answering this question, we should first think about what happens during reconstruction.

During training, the decoders are trained to minimize a reconstruction (typically L1 or L2) loss between the inputs $\{\bs, \bt\}$  and their associated reconstructions $\{f(\z), g(\z)\}$, with $f$ and $g$ being the decoding functions.
%
In a situation where we are only presented with $\bs$, we would still like to obtain the same reconstruction loss for this modality as when we are presented with $\bs$ \emph{and} $\bt$.
%
To do so, we require that the latent code $\z$ remains constant, regardless of whether the other modality is present.
%
Consequently, we need a mechanism to ensure that the encoding distribution is unchanged, regardless of whether the other modality is observed.

Given that we require the latent codes to be unchanged when we have a partially observed modality, we now have to ask the question how we ensure that this remains the case in the situation where both modalities are observed.
%
In this situation, we want to ensure that we are able to reconstruct $\bs$ \emph{and} $\bt$ from $\z \sim q(\z|\bs)$ or $\z \sim q(\z|\bt)$.
%
This can be viewed as the case where we have a single encoder for a VAE and two decoders, that is we encode from one modality and then decode to \emph{both} modalities.
%
From this, we can then repeat the process using the other encoder.
%
An objective of this form would look something like
%
\begin{align}\label{eq:example}
	\E_{q(\z|\bs)}\log\frac{p(\bs|\z)p(\bt|\z)p(\z)}{q(\z|\bs)} + \E_{q(\z|\bt)}\log\frac{p(\bt|\z)p(\bs|\z)p(\z)}{q(\z|\bt)}.
\end{align}
%
Here we are forcing both decoders to directly reconstruct from a sample from only a single posterior.
%
Consequently, when observing a single modality at test time, the decoders should be able to reconstruct both modalities as they have been explicitly optimized to do just that.
%
Conversely, when using an explicit joint distribution function, the decoders are never presented with a latent code that is sampled from the distribution for a single modality, so never learn to reconstruct with missing modalities.
%
We provide the graphical model for this approach in \cref{fig:model}, which demonstrates a swapping of the arrows for one of the modalities.

% \begin{figure}[h]
% 	\centering
% 	\begin{tabular}{cc}
% 		\begin{tikzpicture}
% 		\tikzstyle{main}=[circle, minimum size = 10mm, thick, draw =black!80, node distance = 16mm]
% 		\tikzstyle{connect}=[-latex, thick]
% 		\tikzstyle{box}=[rectangle, draw=black!100]
% 		\node[main, fill = black!10] (s) [label=center:$\bs$] { };
% 		\node[main] (z) [below=of s, label=center:$\z$] { };
% 		\node[main, fill = black!10] (t) [right=of z, label=center:$\bt$] { };
% 		\path (s) edge [dashed, connect, bend right] (z)
% 		(z) edge [dashed, connect, bend right] (t)
% 		(z) edge [connect, bend right] (s)
% 		(t) edge [connect, bend right] (z);
% 		\end{tikzpicture}
% 		&
% 		\begin{tikzpicture}
% 		\tikzstyle{main}=[circle, minimum size = 10mm, thick, draw =black!80, node distance = 16mm]
% 		\tikzstyle{connect}=[-latex, thick]
% 		\tikzstyle{box}=[rectangle, draw=black!100]
% 		\node[main, fill = black!10] (s) [label=center:$\bs$] { };
% 		\node[main] (z) [below=of s, label=center:$\z$] { };
% 		\node[main, fill = black!10] (m) [right=of z, label=center:$\bt$] { };
% 		\path (s) edge [dashed, connect, bend right] (z)
% 		(t) edge [dashed, connect, bend right] (z)
% 		(z) edge [connect, bend right] (s)
% 		(z) edge [connect, bend right] (t);
% 		\end{tikzpicture}
% 	\end{tabular}
% 	\caption{Left: Proposed approach. Right: Mutli-modal VAE~\cite{Wu2018b, Shi2019, sutter2020multimodal}}
% 	\label{fig:model}
% \end{figure}

This purely conceptual approach provides no way to ensure that the encoding distributions actually match, given sufficient capacity in the decoders, they may learn `look-up' style embeddings with the distributions for each modality being completely disjoint.
%
Given that we want to ensure that the encoding distributions for each modality are as close as possible, we subsequently need some mechanism to ensure this.
%
One way to achieve this would be to simply minimize a divergence metric between the two encoding distributions, which will consequently encourage them to have high densities in similar regions of the latent space.

Of course, all of the points outlined in this section are purely conceptual.
%
But from this, we outline two key requirements that we need to satisfy if we are to faithful handle the case where the modalities are partially observed, namely:
%
\begin{enumerate}
	\item Both decoders must be able to reconstruct the data given a sample from \emph{either} encoder.
	\item The encoding distributions must be close according to a distance metric for data points with the same abstract class.
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 2relatedwork_v1.tex <==
\section{Background}\label{sec:background}

Past work on multimodal \glspl{VAE} can be summarised into two categories, based on whether latent samples that contains information from all modalities can be directly obtained or not.

\textbf{Joint latent}:
%
the latent sample obtained from joint posterior $\z \sim q_\Phi(\z | \bs, \bt)$ contains information from both modalities $\bs$ and $\bt$.
%
Early work in multimodal \glspl{VAE} such as  JMVAE \citep{JMVAE_suzuki_1611}, triple ELBO \citep{TELBO_vedantam_1705} and MFM \citep{tsai2018learning} learn a multimodal posterior $q_\Phi(\z|\bs,\bt)$ by defining a single joint encoder that takes concatenated multimodal data as inputs.
%
This line of approaches often requires training auxiliary unimodal components to handle missing modality at test time, and the joint encoder cannot be trained without clean, complete multimodal data.

With MVAE, \citet{Wu2018b} propose to model the joint posterior as a \gls{PoE} of unimodal posteriors.
%
Due to the precision miss-calibration issue of \gls{PoE}, the model \emph{must} be trained with a combination of complete/incomplete multimodal data if it is to handle missing modalities at test time, making the model restrictive in its handling of missing data.
%
In recent work, \citet{gong21} propose VSAE where the joint latent, $\z$, is constructed by concatenating latent samples from unimodal encoders.
%
Inspired by \glspl{VAE} that deal with pixel-level imputation such as VAEAC \citep{ivanov2019variational}, Partial \gls{VAE} \citep{ma2018eddi}, MIWAE \citep{mattei2019miwae} and HI-VAE \citep{nazabal2020handling}, VSAE handles missing modalities at train time by considering a modal-level mask in the graphical model.
%
This however, introduces extra components to the model such as collective proposal network and mask generative network.

One key disadvantage of explicit models is their inability to deal with missing data at train/test time without some form of auxiliary component --- either by training unimodal \glspl{VAE} on the side \citep{JMVAE_suzuki_1611, TELBO_vedantam_1705, tsai2018learning}, train time subsampling \citep{Wu2018b} or modelling of modal-level mask \citep{gong21}.
%
Our proposed model, \gls{MEME}, on the other hand, requires no extra components to handle missing data during train/test.

\textbf{Disjoint latent}:
%
Implicit models describe the scenario where either the joint posterior is not explicitly defined, or the latent sample obtained from the joint posterior does not contain information from both modalities.
%
Examples in this category includes MMVAE proposed by \citet{Shi2019}, which uses \gls{MoE} as factorisation of joint posterior to ameliorate the shortcomings of precision miscalibration in MVAE.
%
More recently, \citet{sutter2021generalized} proposed to combine the two approaches in MoPoE-VAE and demonstrating good results on datasets where the number of modalities involved is greater than 2.
%
In contrast to these methods, mmJSD \citep{sutter2020multimodal} does not define a joint posterior at all---%
instead, the use a dynamic prior is suggested, which is defined as a function $f$ of the unimodal approximated posteriors $q_\phi$ as well as pre-defined prior distribution $p(\z)$.
%
By doing so, the model is able to learn common factors between multiple modalities.

While implicit models cannot produce a joint representation, as a result they also do not need extra components to deal with missing data at test time. %
However, all work listed above requires complete multimodal data to train properly.
%
Our proposed method also belongs in the category of implicit model, however, it benefits from a semi-supervised learning perspective and can be trained with incomplete multimodal data.



\begin{table}[h]
	\centering
	\caption{We examine 4 characteristics of each model, including whether the model can handle missing modalities during 1) test and 2) train, 3) form of joint posterior (or latent sample) in the bi-modal case and 4) extra components. (\cmark) indicates theoretical capability that is not verified empirically.}
	{\small
		\begin{tabular}{lcccc}
			\toprule
			& Missing Test & Missing Train & Joint posterior & Extra Component\\
			\midrule
            JMVAE & \cmark & \xmark & $q_\Phi(\z|\bs,\bt)$ & $q_{\phi_s}(\z|\bs),q_{\phi_t}(\z|\bt)$\\
            tELBO & \cmark & \xmark & $q_\Phi(\z|\bs,\bt)$ & $q_{\phi_s}(\z|\bs),q_{\phi_t}(\z|\bt)$\\
            MFM   & \cmark & \xmark & $q_\Phi(\z|\bs,\bt)$ & $q_{\phi_s}(\z|\bs),q_{\phi_t}(\z|\bt)$\\
            MVAE  & \cmark & (\cmark) & $q_{\phi_s}(\z|\bs)q_{\phi_t}(\z|\bt)p(\z)$ & sub-sampling\\
            MMVAE & \cmark & \xmark & $q_{\phi_s}(\z|\bs) + q_{\phi_t}(\z|\bt)$ & -\\
            MoPoE & \cmark & (\cmark) & $q_{\phi_s}(\z|\bs)+q_{\phi_t}(\z|\bt)+q_{\phi_s}(\z|\bs)q_{\phi_t}(\z|\bt)$ & -\\
            VSVAE & \cmark & \cmark & \texttt{concat}$(z_s, z_t)$ & - \\
            mmJSD & \cmark & \xmark & - & -\\
            \textbf{Ours} & \cmark & \cmark & - & - \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:comparison}
\end{table}












% Several works have attempted to address these shortcomings.
% %
% \citet{Wu2018b} adopt a sub-sampling scheme to handle missing data at test time and use the \gls{ELBO} for single modalities on top of the original joint \gls{ELBO}.
% %
% This allows the model to deal with occasional missing data during train time, however, as we show in experiment the sub-sampling scheme is not only cumbersome, but also ineffective for large amount of missing data.
% %
% %
% \citet{shi2021relating} propose a contrastive \gls{ELBO} for multimodal \glspl{VAE} which aims at reducing the amount of paired data needed by learning the \enquote{relatedness} between datapoints.
% %
% However, their objective is not able to deal with partially observed case.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 4experiment_v1.tex <==
% Sid's comments:

% This section needs an involved edit pass to make sure that it tells a _story_.
% Right now, it reads heavily like a collection of observations from an lab notebook.

% The section needs an 'introduction'
% The narrative in it needs to lead the reader, gently, into
% - what we aim to do (standard evaluation, cite relevant paper that do it)
% - oh look there's something extra we can do---because the model enables it, partial-observations!
% - what these evaluations will be run on, and why (because others do it, and it challenging...)
% - also, with the _implicit_ combination we do, and the ability to learn from partial data
%   + what can we probe about the representations learnt?
%   + we look at whether there is any indication of discriminative information in the latent about whether data is related.
%   + we also compare to see if other/baselines capture anything similar.

% Then we can setup the different subsections to go into details of the experiments themselves.
% For each subsection
% - explain/reiterate what it's doing
%   if coherence, say what it is and what it measures
% - provide details on train/test and hyperparameter choices
% - present results and discuss them

% Results:
% - convert partial-supervision tables into graphs
% - simplify/shrink 4.2 and the distance matrix plots
% - add back the classifier tables and the qualitiatve results for cub

\section{Experiments}
%
Following the contributions of \gls{MEME}, we seek to examine the ability of our model to perform in the partially observed training regime~(\cref{sec:partial}); but also its ability to extract a notion or relatedness between samples~(\cref{sec:relatedness}).
%
The experiments provided in the main paper are designed to highlight the above, but we  include further experiments associated with multimodal VAEs in the appendix. %\cref{app:results}.
%
Evaluations are performed on a paired version of MNIST~\citep{lecun2010mnist} and SVHN~\citep{netzer2011reading}, as well as the more challenging CUB dataset~\citep{WelinderEtal2010}, with the data modalities representing an image and caption.
%
For image modalities we utilize a Laplacian likelihood and a Categorical likelihood for text, with the distributions on the latent space being parameterized by Gaussians.
%
We find that increasing the strength of the classifier in \cref{eq:ccvae} ($\qts$), aides training, and chose a multiplicative value of 10 as it worked well in practice.


\subsection{Partially Observed Training}\label{sec:partial}
%
Here we demonstrate the main contribution of our approach --- evaluating the models performance in training regimes where either of the modalities are partially observed.
%
Specifically, for each modality, we partially observe the other during training for a given fraction $f$ of the data.
%
The modality which is present all of the time is indicated in subscript to the method,
%
e.g, \gls{MEME}\textsubscript{MNIST} with $f = 0.25$ indicates that only 25\% of samples are paired, and the other 75\% only contain MNIST digits.
%
We perform this partial observations for each modality, allowing us to observe the effects that fully observing each modality has.
%
Training was performed on five observation rates of $100\%, 50\%$, $25\%$, $12.5\%$ and $6.25\%$, for the case where MNIST and SVHN are missing respectively, and $100\%, 50\%$ and $25\%$ for CUB.
%
It is important to note that MMVAE can only be trained in the fully observed case, due to the choice of MoE in the posterior.

The main utility of multi-modal VAEs arises in their ability to perform domain adaptation, or transfer an underlying abstract concept from one modality to another.
%
Here we focus primarily on the models ability to cross-generate samples, that is given a modality $\bs$, generate a $\bt$.
%
Consequently, the results provided in this section act as an indicator of the models performance to perform cross-generation.
%
However, we also report more experiments relating to the generative quality, and performance on downstream tasks in~\cref{app:results}.
%
Following previous work~\cite{Shi2019}, we evaluate the models using the coherence score for MNIST-SVHN and a correlation values for CUB.

\begin{figure}
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\begin{tabular}{@{}r@{\s}c@{\r}|c@{\r}}
%		&\multicolumn{2}{c}{\gls{MEME}}& \multicolumn{2}{c}{\gls{MEME}}\\
		Input Image & \includegraphics[width=0.2\linewidth]{media/friday/mnist.png} & \includegraphics[width=0.2\linewidth]{media/friday/svhn.png} \\
		Cross Generations & \includegraphics[width=0.2\linewidth]{media/friday/ccvae_mnist_to_svhn.png} & \includegraphics[width=0.2\linewidth]{media/friday/ccvae_svhn_to_mnist.png}
	\end{tabular}\caption{Cross Generations from \gls{MEME}, here we take the input image (top row) and perform a cross generation to obtain the bottom row.}
\end{figure}


\paragraph{Coherence Scores}
%
Following~\citet{Shi2019}, we report the coherence scores for cross-generation.
%
The coherence score indicates how often a pre-trained classifier obtains the correct prediction given a cross-generation and the corresponding label to its source.
%
This metric provides a quantitative measure into the quality of the cross-generations\footnote{we also provide additional results into how `in-distribution' the generations are in \cref{app:results}.}.
%
As we can see in \cref{tab:coherence}, our model is able to obtain superior coherence scores in the fully observed and partially observed case.
%
It is interesting to see that cross-generating MNIST (bottom table) obtains a similar performance depending on whether we partially observe MNIST of SVHN.
%
We posit that this is due to the information needed to generate an MNIST digit is typically sub-summed within an SVHN digit (e.g. there is little style information associated with MNIST), consequently making generation easier.
%
The same is not true for MNIST $\rightarrow$ SVHN, where we see a dramatic decrease in coherence scores when partially observing MNIST.
%
We hypothesize that this is due to a natural discord between the clustering of MNIST and SVHN, of which the former requires fewer modes---typically one per class.
%
Consequently, we are not able to encode the MNIST digit into a region of the latent space which the SVHN decoder can reconstruct from.

\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Coherence Scores for MNIST $\rightarrow$ SVHN (Top) and for SVHN $\rightarrow$ MNIST (Bottom). Subscript indicates which modality is always present during training, $f$ indicates the percentage of matched samples. Higher is better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			& \multicolumn{5}{c}{MNIST $\rightarrow$ SVHN}\\
			\cmidrule(r{12pt}){2-6}
			Model & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ & $f = 0.0625$  \\
			\midrule
			\gls{MEME}\textsubscript{SVHN} & \textbf{0.625 $\pm$ 0.007} & \textbf{0.551 $\pm$ 0.008} & \textbf{0.323 $\pm$ 0.025}        & \textbf{0.172 $\pm$ 0.016}  &   \textbf{0.143 $\pm$ 0.009} \\
			MMVAE\textsubscript{SVHN} & 0.581 $\pm$ 0.008 & - & - & - & - \\
			MVAE\textsubscript{SVHN} &  0.123 $\pm$ 0.003 & 0.110 $\pm$ 0.014        &      0.112 $\pm$ 0.005        &      0.105 $\pm$ 0.005        &   0.105 $\pm$ 0.006 \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{MNIST}  & \textbf{0.625 $\pm$ 0.007}  & \textbf{0.572 $\pm$ 0.003}  & \textbf{0.485 $\pm$ 0.013} & \textbf{0.470 $\pm$ 0.009} &  \textbf{0.451 $\pm$ 0.011} \\
			MMVAE\textsubscript{MNIST}  & 0.581 $\pm$ 0.008 & - & - & - & -  \\
			MVAE\textsubscript{MNIST} & 0.123 $\pm$ 0.003        &       0.111 $\pm$ 0.007        &      0.112 $\pm$ 0.013        &      0.116 $\pm$ 0.012        &      0.116 $\pm$ 0.005  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{SPLIT} & - & 0.625 $\pm$ 0.008        &       0.503 $\pm$ 0.008        &      0.467 $\pm$ 0.013        &      0.387 $\pm$ 0.010 \\
			MVAE\textsubscript{SPLIT} & - & - \\
			\cmidrule(r{12pt}){2-6}\\
			& \multicolumn{5}{c}{SVHN $\rightarrow$ MNIST}\\
			\cmidrule(r{12pt}){2-6}
			Model & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ & $f = 0.0625$ \\
			\midrule
			\gls{MEME}\textsubscript{SVHN} & \textbf{0.752 $\pm$ 0.004}   & \textbf{0.726 $\pm$ 0.006}        &      \textbf{0.652 $\pm$ 0.008}        &      \textbf{0.557 $\pm$ 0.018}  &   \textbf{0.477 $\pm$ 0.012}  \\
			MMVAE\textsubscript{SVHN}  & 0.735 $\pm$ 0.010 &  - & - & - & -   \\
			MVAE\textsubscript{SVHN}  & 0.213 $\pm$ 0.004 & 0.174 $\pm$ 0.061        &      0.148 $\pm$ 0.018        &      0.116 $\pm$ 0.013        &   0.109 $\pm$ 0.002  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{MNIST} & \textbf{0.752 $\pm$ 0.004}        &       \textbf{0.715 $\pm$ 0.003}        &      \textbf{0.603 $\pm$ 0.018}        &      \textbf{0.546 $\pm$ 0.012}        &      \textbf{0.446 $\pm$ 0.008}   \\
			MMVAE\textsubscript{MNIST} & 0.735 $\pm$ 0.010 & - & - & - & -  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{SPLIT} & - & 0.718 $\pm$ 0.002        &       0.621 $\pm$ 0.007        &      0.568 $\pm$ 0.014        &      0.503 $\pm$ 0.001 \\
			MVAE\textsubscript{SPLIT} & - & - \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:coherence}
\end{table}

\paragraph{Canonical Correlation Analysis:}
%
To provide a quantitative metric for the efficacy of our modal on CUB, we report the correlation between cross-generations using Canonical Correlation Analysis (CCA), which has previously been utilized for image caption data~\citet{massiceti2018visual, Shi2019}.
%
% Specifically, given two observation $\{\x_1 \in \mathbb{R}^n_1, \x_2 \in \mathbb{R}^n_2\}$, CCA learns the projections $W_1 \in \mathbb{R}^{n_1 \times m}$ and $W_2 \in \mathbb{R}^{n_2 \times m}$ which maximize the correlation between the projections $W_1^T\x_1$ and $W_2^T\x_2$.
% %
% The correlation between observations can thus be computed as the cosine distance between the mean-centered projections:
% %
% \begin{align}
% \text{corr}(\x_1, \x_2) = \frac{\phi(\x_1)^T\phi(\x_2)}{||\phi(\x_1)||_2||\phi(\x_2)||_2},
% \end{align}

% with $\phi(\x_i) = W_i^T\x_i - \E_i[W_i^T\x_i]$.
% %
% We follow~\citet{Shi2019} by treating $\x_1$ and $\x_2$ as the ResNet-101 image features and a 300-d projection~\citet{bojanowski2016enriching} for the captions.
%
We report the correlations for cross generations in \cref{tab:corr} and also prove qualitative results in the Appendix.
%
Where we can see that \gls{MEME} is consistently better than MVAE accross all supervision rates, and better than MMVAE in the fully supervised case.
%
Generally, cross-generating images yields higher correlation values, possibly due to the difficulty in generating semantically meaningful text.
%
% We would like to highlight that typically, fully observing captions yields similar correlation values for Image $\rightarrow$ Caption and Caption $\rightarrow$ Image, which is not the case when fully observing images.
% %
% In this instance, the correlations when cross-generating a caption yields lower values---possibly due to the difficulty in generating semantically meaningful text.
We would like to highlight that typically fully observing images leads to poorer performance when cross-generating captions.
%
Again, possibly due to the difficulty in generating text, but also possibly due to a discord between how the latent space is structured, where a similar pattern emerged when MNIST was only partially observed.
%



\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Correlation Values for CUB cross generations. Higher is better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			& \multicolumn{5}{c}{Image $\rightarrow$ Captions}\\
			\cmidrule(r{12pt}){2-6}
			Model & GT & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ \\
			\midrule
			\gls{MEME}\textsubscript{Image} & {0.106 $\pm$ 0.000} & \textbf{0.064 $\pm$ 0.011} & \textbf{0.042 $\pm$ 0.005} & \textbf{0.026 $\pm$ 0.002} & \textbf{0.029 $\pm$ 0.003}\\
			MMVAE\textsubscript{Image} & 0.106 $\pm$ 0.000 & 0.060 $\pm$ 0.010 & - & - & - \\
			MVAE\textsubscript{Image} & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001 & -0.000 $\pm$ 0.004       &      0.001 $\pm$ 0.004        &      -0.001 $\pm$ 0.005 \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & \textbf{0.064 $\pm$ 0.011}  & \textbf{0.062 $\pm$ 0.006} & \textbf{0.048 $\pm$ 0.004} & \textbf{0.052 $\pm$ 0.002} \\
			MMVAE\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & 0.060 $\pm$ 0.010 & - & - & -  \\
			MVAE\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001       &       -0.000 $\pm$ 0.004       &      0.000 $\pm$ 0.003        &      0.001 $\pm$ 0.002   \\
			\cmidrule(r{12pt}){2-6}\\
			& \multicolumn{5}{c}{Caption $\rightarrow$ Image}\\
			\cmidrule(r{12pt}){2-6}
			Model & GT & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ \\
			\midrule
			\gls{MEME}\textsubscript{Image} & 0.106 $\pm$ 0.000 & \textbf{0.074 $\pm$ 0.001} & \textbf{0.058 $\pm$ 0.002} &      \textbf{0.051 $\pm$ 0.001}  & \textbf{0.046 $\pm$ 0.004}  \\
			MMVAE\textsubscript{Image}  & 0.106 $\pm$ 0.000 & 0.058 $\pm$ 0.001 & - & - & -   \\
			MVAE\textsubscript{Image}  & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001 & -0.002 $\pm$ 0.000       &      -0.002 $\pm$ 0.001       &      -0.001 $\pm$ 0.001  \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{Captions} & 0.106 $\pm$ 0.000 & \textbf{0.074 $\pm$ 0.001} & 0\textbf{.059 $\pm$ 0.003} & \textbf{0.050 $\pm$ 0.001} & \textbf{0.053 $\pm$ 0.001}   \\
			MMVAE\textsubscript{Captions} & 0.106 $\pm$ 0.000 & 0.058 $\pm$ 0.001 & - & - & -  \\
			MVAE\textsubscript{Captions} & 0.106 $\pm$ 0.000 & 0.002 $\pm$ 0.001       &       -0.001 $\pm$ 0.002       &      -0.003 $\pm$ 0.002       &      -0.002 $\pm$ 0.001 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:corr}
\end{table}

\paragraph{Discussion} In this sub-section we outlined how \gls{MEME} is able to obtain good performance on cross-generation tasks when partially observing either modality.
%
One key result from theses experiments is the in-balance between results depending on which modality is observed, e.g. partially observing MNIST leads to poor cross-generations for MNIST $\rightarrow$ SVHN and partially observing captions leads to poor cross-generations for Image $\rightarrow$ Captions.
%
Hypothetically, this is not an unsurprising result, as the objective used here has been shown to structure the latent space~\citep{joy2021capturing} depending on the information from the other modalities, i.e. in their work they used labels enforce disentanglement of the latent factors.
%
Consequently, the structure of the latent space will change depending on which modality is partially observed, which in turn will have a subsequent knock-on effect on the generations.
%
We further investigated this effect in \cref{app:results}, where we also present additional results on the performance of \gls{MEME}, but omitted them to the Appendix due to space constraints.

\subsection{Extracting Relatedness}\label{sec:relatedness}
%
% In this section, we examine our model's capability to capture relatedness in its latent space.
%
% As a result of the mutual supervision aspect of our objective, we can directly use the distance between the encoding distributions of different modalities as a measure of ``relatedness''.
%
% Intuitively, the smaller the distance is, the more likely the given data pairs are related.
%
% This could help us identify paired multimodal samples from unlabelled datasets, which could potentially be used for further training of the generative model.

%
One of the key advantages of our approach is that a mechanism for extracting relatedness between samples naturally emerges.
%
Because during training we regularize the encoding distributions to be near to each other when they are encoding a data-point with of a similar abstract concept, at test time we can compare the closeness of these distributions to extract a metric for relatedness.
%
Here we use the 2-Wasserstein distance --- a symmetric metric with closed form expression (see Appendix for more details).
%\cref{app:wassertein}
Specifically, we compute $d_{ij} = \calW_2(q(\z|\bs_i)||q(\z|\bt_j))$, where $q(\z|\bs_i)$ and $q(\z|\bt_j)$ are the individual encoders, for all combination of pairs $\{\bs_i, \bt_j\}$ in the mini-batch, i.e $\{\bs_i, \bt_j\} \in \mathcal{B}~\forall~i,~j\in\{1\dots ,M\}$ where $M$ is the number of elements in the mini-batch $\mathcal{B}$.
%
We then plot $d_{ij}$ on a histogram, and we color-code the histogram by whether the corresponding data pair $\{\bs_i, \bt_j\}$ are related.
%
Ideally, we should observe smaller distances between encoding distributions for data pairs that are related, and larger for the ones that are not.

% From this data, we can then construct two histograms which indicate the distribution of the distances for pairs which are matched and pairs which are not.
%
% Intuitively, a model which extracts relatedness successfully should have a higher mass for closer distances and lower mass for further distances when the samples \emph{are} related.
%
% The opposite is true for when they are not related, i.e. we should see a high mass at further distances.

See results in \cref{fig:histograms}.
%
We see that \gls{MEME} generally yields a higher mass at lower distance values for the matched case than it does for the unmatched case, indicating a high probability of closer distances when pairs are matched than when they are not.
%
MMVAE goes someway to obtaining a similar pattern, but falls short of achieving the same disparity as \gls{MEME}, the distributions for MVAE match completely, indicating a complete inability to extract relatedness.



\begin{figure}[h!]
	\centering
	\scalebox{0.9}{
	\begin{tabular}{ccc}
		\includegraphics[width=0.33\linewidth]{media/friday/ccvae_digits_histogram.png}&
		\includegraphics[width=0.33\linewidth]{media/friday/mmvae_digits_histogram.png}&			\includegraphics[width=0.33\linewidth]{media/friday/mvae_digits_histogram.png}	\\
		\includegraphics[width=0.33\linewidth]{media/friday/ccvae_cub_histogram.png}&
		\includegraphics[width=0.33\linewidth]{media/friday/mmvae_cub_histogram.png}&			\includegraphics[width=0.33\linewidth]{media/friday/mvae_cub_histogram.png}
	\end{tabular}
	}
	\caption{Histograms of Wassertein distance for SVHN and MNIST (Top) and CUB (Bottom): Ours (Left), MMVAE (middle) and MVAE (Right). Blue indicates unmatched samples and orange matched samples. We expect to see high densities of blue at further distances and visa-versa for orange.}
	\label{fig:histograms}
\end{figure}


\subsubsection{Multi-class distance Matrix}
%
For the MNIST-SVHN case, we can extract relatedness on a per-class basis.
%
To do this, we construct a distance matrix for the classes $\mathbf{K}\in\mathbb{R}^{10\times10}$, with each element corresponding to the average $\calW_2$ distance between encoding distributions of the corresponding classes.
%
I.e. for each batch, $K_{\{u, v\}} = \sum_{i\in\mathcal{I}}\sum_{j\in\mathcal{J}}d_{ij}~\text{s.t.}~\mathcal{I}=\{i \in \{1,\dots,M\}|\y_i = u\},~\mathcal{J}=\{j \in \{1,\dots,M\}|\y_j = v\}$, with $\y$ representing the class labels and then subsequently taking the average.
%
A perfect distance matrix will consist of a diagonal of all zeros and positive values in the off-diagonal.

We display distance matrices, for the fully matched case in \cref{fig:confusion_mat}, where it can be seen that in general our method produces a lower diagonal, and a higher average distance for the off-diagonals.
%
MMVAE also obtains a lower diagonal, but also provides lower values for the off diagonals, MVAE is completely unable to extract relatedness.

Inspecting the confusion matrices further, we see some interesting features.
%
For instance, our model is able to extract the understanding that SVHN \texttt{3} is similar to MNIST \texttt{5} and \texttt{8} (fourth column), and that \texttt{1} and \texttt{0} are completely unrelated.
%
A similar pattern can be seen in MMVAE, but again this is not as pronounced and MVAE completely fails in this case.
%
To further extract this structure, we construct a dendrogram to visualize the hierarchical clustering of the relatedness, which we display in \cref{fig:confusion_mat}.
%
Again we see that our model is able to obtain a clustering which one would typically associate with a digit dataset.
%
E.g. \texttt{3}, \texttt{5} and \texttt{8} cluster together, along with \texttt{6} and then \texttt{9}, typically we see a clustering of digits which tend to have a smooth writing profile (e.g. \texttt{8}), before the clustering of digits with sharp angles, with \texttt{0} and \texttt{1} being the most different.
%
This is not the case for MMVAE, which seems to cluster in a different manner, and again MVAE completely fails.
%
It is also important to note the values at which the clustering occurs, a higher value indicated a much greater distance between clusters.
%
Generally the clusters obtained in \gls{MEME} are separated further apart than for MMVAE, indicated by higher values on the y axis of the dendrogram.


\begin{figure}[h!]
	\centering
	\scalebox{0.8}{
	\begin{tabular}{ccc}
		\includegraphics[width=0.3\linewidth]{media/friday/ccvae_confusion_mat.png}&
		\includegraphics[width=0.3\linewidth]{media/friday/mmvae_confusion_mat.png}&			\includegraphics[width=0.3\linewidth]{media/friday/mvae_confusion_mat.png}\\
		\includegraphics[width=0.3\linewidth]{media/friday/ccvae_dendrogram.png}&
		\includegraphics[width=0.3\linewidth]{media/friday/mmvae_dendrogram.png}&			\includegraphics[width=0.3\linewidth]{media/friday/mvae_dendrogram.png}
	\end{tabular}
	}
	\caption{Distance matrices for KL divergence between classes for SVHN and MNIST (Top) and dendrogram (Bottom) for: Ours (Left), MVAE (middle) and MMVAE (Right).}
	\label{fig:confusion_mat}

\end{figure}

To further quantify the relatedness numerically, we report the correlation coefficient for each distance matrix.
%
Specifically, we treat the dimensions of the matrix as random variables and the entries as pseudo probabilities of relatedness.
%
This then allows us to compute the sample correlation coefficient between the modalities.
%
For further information please see \cref{app:corr_coef}.
%
We present these results in \cref{tab:cond_number}, where we see that we are consistently able to report high correlation values, indicating that our method is able to extract relatedness, even in that partially observed case.
%
\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Correlation Coefficient of Confusion Matrices. Higher is Better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			Model & $1.0$ & $0.5$ & $0.25$ & $0.125$ & $0.0625$ \\
			\midrule
			Ours\textsubscript{SVHN} & \textbf{0.493 $\pm$ 0.020}  & \textbf{0.238 $\pm$ 0.011} & \textbf{0.110 $\pm$ 0.005} & \textbf{0.055 $\pm$ 0.013} & \textbf{0.030 $\pm$ 0.009} \\
			MMVAE\textsubscript{SVHN} & 0.477 $\pm$ 0.013 & - & - & - & \\
			MVAE\textsubscript{SVHN} & -0.018 $\pm$ 0.021 & -0.005 $\pm$ 0.012 & 0.005 $\pm$ 0.060 & -0.002 $\pm$ 0.014  & 0.000 $\pm$ 0.002 \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{MNIST} & \textbf{0.493 $\pm$ 0.020}  & \textbf{0.190 $\pm$ 0.012} & \textbf{0.084 $\pm$ 0.003} & \textbf{0.059 $\pm$ 0.005}  & \textbf{0.044 $\pm$ 0.003}  \\
			MMVAE\textsubscript{MNIST} & 0.477 $\pm$ 0.013 & - & - & - & - \\
			MVAE\textsubscript{MNIST} & -0.018 $\pm$ 0.021  & -0.002 $\pm$ 0.005 & 0.000 $\pm$ 0.001 & nan $\pm$ nan & nan $\pm$ nan \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:cond_number}
\end{table}


%\subsection{Complex Dataset}
%%
%We now turn out attention to the more complex dataset, CUB~\citet{WelinderEtal2010}, which consists of 11,788 photograph of birds in a variety of different natural scenes.
%%
%Each photograph is accompanied by 10 fine-grained captions, describing the features of the bird, (e.g. crown color, beak size, etc.), caption were generated by humans through Amazon Mechanical Turk.
%%
%An example image and caption is given in \cref{fig:cub_ex}.
%%
%Following~\citet{Shi2019}, we treat the image features as one modality and the captions as the other, avoiding blurry image generations~\citet{zhao2017towards}.
%%
%Features are extracted from an off-the-shelf pre-trained ResNet-101 network~\citet{resnet}.
%%
%To obtain a reconstructed image, we perform nearest neighbor lookup in the feature space using the reconstructed feature.
%%
%We utilize a CNN networks for text modality~\citet{kalchbrennerconvolutional, pham2016convolutional, massiceti2018}, and a Categorical distribution for the likelihood function.
%



% \begin{figure}
% 	\begin{tabular}{C{1.0cm}  L{11.5cm}}
% 		\includegraphics[width=\linewidth]{media/friday/cub/ccvae/image_7.png} &
% 		\texttt{<sos> this bird has a blue head and back, an orange breast, and cream wingbars lined with black coverts. <eos>}
% 	\end{tabular}
% 	\caption{Example CUB image and associated caption.}
% 	\label{fig:cub_ex}
% \end{figure}








%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/1.0/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $100\%$.}
%	\label{fig:embeddings_sup}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.5_a/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $50\%$ drop rate SVHN.}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.1_a/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $10\%$ drop rate SVHN.}
%\end{figure}
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.5_b/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $50\%$ drop rate MNIST.}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.1_b/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $10\%$ drop rate MNIST.}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 4experiments_v2.tex <==
% Sid's comments:

% This section needs an involved edit pass to make sure that it tells a _story_.
% Right now, it reads heavily like a collection of observations from an lab notebook.

% The section needs an 'introduction'
% The narrative in it needs to lead the reader, gently, into
% - what we aim to do (standard evaluation, cite relevant paper that do it)
% - oh look there's something extra we can do---because the model enables it, partial-observations!
% - what these evaluations will be run on, and why (because others do it, and it challenging...)
% - also, with the _implicit_ combination we do, and the ability to learn from partial data
%   + what can we probe about the representations learnt?
%   + we look at whether there is any indication of discriminative information in the latent about whether data is related.
%   + we also compare to see if other/baselines capture anything similar.

% Then we can setup the different subsections to go into details of the experiments themselves.
% For each subsection
% - explain/reiterate what it's doing
%   if coherence, say what it is and what it measures
% - provide details on train/test and hyperparameter choices
% - present results and discuss them

% Results:
% - convert partial-supervision tables into graphs
% - simplify/shrink 4.2 and the distance matrix plots
% - add back the classifier tables and the qualitiatve results for cub

\section{Experiments}
%
Here we seek to examine the ability of \glspl{MEME} performance on standard benchmarks for multi-modal VAEs against the baselines of MVAE and MMVAE.
%
Specifically, we are primarily focused on the \emph{partially observed} training regime, where either or both of the modalities may be partially observed during training.
%
Following previous work~\citep{Shi2019, sutter2020multimodal, sutter2021generalized}, we use the standard benchmark of coherence~(\cref{sec:coherence}) and also investigate the structure of the learnt latent space through a discriminative classification task~(\cref{sec:disc}).
%
Evaluating the coherence provides an indication into how well the model can cross-generate samples, whilst the discriminative task provides an intuition into the interpreability of the latent representation and its use for downstream tasks.

Due to the formulation of our approach, we also see the emergence of a natural mechanism for extracting relatedness between a sample from each modality.
%
That is, given a sample from each modality, can we obtain a metric into how similar these samples are in a conceptual sense?
%
Our method is able to do just that, and we extensively evaluate its ability to do so by providing informative figures on the relatedness of the samples~(\cref{sec:relatedness}).


The experiments provided in the main paper are designed to highlight the above, but we include further experiments associated with multimodal VAEs in the appendix. %\cref{app:results}.
%
Evaluations are performed on a paired version of MNIST~\citep{lecun2010mnist} and SVHN~\citep{netzer2011reading}, as well as the more challenging CUB dataset~\citep{WelinderEtal2010}, with the data modalities representing an image and caption.
%
For each data-set we constructed a separate test split which contained the same samples for all training runs.
%
Training was performed with various observation rates for each modality.
%
Specifically, for each modality, we partially observe the other during training for a given fraction $f$ of the data.
%
The modality which is present all of the time is indicated in subscript to the method,
%
e.g, \gls{MEME}\textsubscript{MNIST} with $f = 0.25$ indicates that only 25\% of samples are paired, and the other 75\% only contain MNIST digits.
%
The subscript SPLIT indicates that each modality was equally partially observed for the remaining of the data.
%
Training was performed on five observation rates of $100\%, 50\%$, $25\%$, $12.5\%$ and $6.25\%$, for the case where MNIST and SVHN are missing respectively, and $100\%, 50\%$ and $25\%$ for CUB.
%
MMVAE was only trained using fully observed data, due to its inability to deal with the partially observed case.

For image modalities we utilize a Laplacian likelihood and a Categorical likelihood for text, with the distributions on the latent space being parameterized by Gaussians.
%
We find that increasing the strength of the classifier in \cref{eq:ccvae} ($\qts$), aides training, and chose a multiplicative value of 10 as it worked well in practice.


\subsection{Evaluating Coherence}\label{sec:coherence}
%
The main utility of multi-modal VAEs arises in their ability to perform domain adaptation, or transfer an underlying abstract concept from one modality to another.
%
Here we focus primarily on the models ability to cross-generate samples, that is given a modality $\bs$, generate a $\bt$.
%
Following~\citet{Shi2019}, we report the coherence scores (MNIST-SVHN) and preform CCA (CUB) on cross-generations.
%
The coherence score indicates how often a pre-trained classifier obtains the correct prediction given a cross-generation and the corresponding label to its source, which provides a quantitative measure into the quality of the cross-generations\footnote{we also provide additional results into how `in-distribution' the generations are in \cref{app:results}.}.


\begin{figure}
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\begin{tabular}{@{}r@{\s}c@{\r}|c@{\r}}
%		&\multicolumn{2}{c}{\gls{MEME}}& \multicolumn{2}{c}{\gls{MEME}}\\
		Input Image & \includegraphics[width=0.2\linewidth]{media/friday/mnist.png} & \includegraphics[width=0.2\linewidth]{media/friday/svhn.png} \\
		Cross Generations & \includegraphics[width=0.2\linewidth]{media/friday/ccvae_mnist_to_svhn.png} & \includegraphics[width=0.2\linewidth]{media/friday/ccvae_svhn_to_mnist.png}
	\end{tabular}\caption{Cross Generations from \gls{MEME}, here we take the input image (top row) and perform a cross generation to obtain the bottom row.}
\end{figure}


\paragraph{MNIST-SVHN} As we can see in \cref{tab:coherence}, our model is able to obtain superior coherence scores in the fully observed and partially observed case.
%
It is interesting to see that cross-generating MNIST (bottom table) obtains a similar performance depending on whether we partially observe MNIST of SVHN.
%
We posit that this is due to the information needed to generate an MNIST digit is typically sub-summed within an SVHN digit (e.g. there is little style information associated with MNIST), consequently making generation easier.
%
The same is not true for MNIST $\rightarrow$ SVHN, where we see a dramatic decrease in coherence scores when partially observing MNIST.
%
We hypothesize that this is due to a natural discord between the clustering of MNIST and SVHN, of which the former requires fewer modes---typically one per class.
%
Consequently, we are not able to encode the MNIST digit into a region of the latent space which the SVHN decoder can reconstruct from.

\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Coherence Scores for MNIST $\rightarrow$ SVHN (Top) and for SVHN $\rightarrow$ MNIST (Bottom). Subscript indicates which modality is always present during training, $f$ indicates the percentage of matched samples. Higher is better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			& \multicolumn{5}{c}{MNIST $\rightarrow$ SVHN}\\
			\cmidrule(r{12pt}){2-6}
			Model & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ & $f = 0.0625$  \\
			\midrule
			\gls{MEME}\textsubscript{SVHN} & \textbf{0.625 $\pm$ 0.007} & \textbf{0.551 $\pm$ 0.008} & \textbf{0.323 $\pm$ 0.025}        & \textbf{0.172 $\pm$ 0.016}  &   \textbf{0.143 $\pm$ 0.009} \\
			MMVAE\textsubscript{SVHN} & 0.581 $\pm$ 0.008 & - & - & - & - \\
			MVAE\textsubscript{SVHN} &  0.123 $\pm$ 0.003 & 0.110 $\pm$ 0.014        &      0.112 $\pm$ 0.005        &      0.105 $\pm$ 0.005        &   0.105 $\pm$ 0.006 \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{MNIST}  & \textbf{0.625 $\pm$ 0.007}  & \textbf{0.572 $\pm$ 0.003}  & \textbf{0.485 $\pm$ 0.013} & \textbf{0.470 $\pm$ 0.009} &  \textbf{0.451 $\pm$ 0.011} \\
			MMVAE\textsubscript{MNIST}  & 0.581 $\pm$ 0.008 & - & - & - & -  \\
			MVAE\textsubscript{MNIST} & 0.123 $\pm$ 0.003        &       0.111 $\pm$ 0.007        &      0.112 $\pm$ 0.013        &      0.116 $\pm$ 0.012        &      0.116 $\pm$ 0.005  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{SPLIT} & - & 0.625 $\pm$ 0.008        &       0.503 $\pm$ 0.008        &      0.467 $\pm$ 0.013        &      0.387 $\pm$ 0.010 \\
			MVAE\textsubscript{SPLIT} & - & 0.108 $\pm$ 0.005        &       0.101 $\pm$ 0.005        &      0.101 $\pm$ 0.001        &      0.101 $\pm$ 0.002 \\
			\cmidrule(r{12pt}){2-6}\\
			& \multicolumn{5}{c}{SVHN $\rightarrow$ MNIST}\\
			\cmidrule(r{12pt}){2-6}
			Model & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ & $f = 0.0625$ \\
			\midrule
			\gls{MEME}\textsubscript{SVHN} & \textbf{0.752 $\pm$ 0.004}   & \textbf{0.726 $\pm$ 0.006}        &      \textbf{0.652 $\pm$ 0.008}        &      \textbf{0.557 $\pm$ 0.018}  &   \textbf{0.477 $\pm$ 0.012}  \\
			MMVAE\textsubscript{SVHN}  & 0.735 $\pm$ 0.010 &  - & - & - & -   \\
			MVAE\textsubscript{SVHN}  & 0.213 $\pm$ 0.004 & 0.174 $\pm$ 0.061        &      0.148 $\pm$ 0.018        &      0.116 $\pm$ 0.013        &   0.109 $\pm$ 0.002  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{MNIST} & \textbf{0.752 $\pm$ 0.004}        &       \textbf{0.715 $\pm$ 0.003}        &      \textbf{0.603 $\pm$ 0.018}        &      \textbf{0.546 $\pm$ 0.012}        &      \textbf{0.446 $\pm$ 0.008}   \\
			MMVAE\textsubscript{MNIST} & 0.735 $\pm$ 0.010 & - & - & - & -  \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{SPLIT} & - & 0.718 $\pm$ 0.002        &       0.621 $\pm$ 0.007        &      0.568 $\pm$ 0.014        &      0.503 $\pm$ 0.001 \\
			MVAE\textsubscript{SPLIT} & - & 0.336 $\pm$ 0.015        &       0.279 $\pm$ 0.003        &      0.249 $\pm$ 0.017        &      0.169 $\pm$ 0.005 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:coherence}
\end{table}

\paragraph{CUB} Due to the lack of classes in CUB, to provide a quantitative metric for the efficacy of our modal on CUB, we instead report the correlation between cross-generations using Canonical Correlation Analysis (CCA), which has previously been utilized for image caption data~\citet{massiceti2018visual, Shi2019}.
%
In a similar vein to coherence, a cross-generation should yield a high correlation between input and the cross generation on a pre-defined feature space if the cross-generation is pertinent in its concept to the input.
%
% Specifically, given two observation $\{\x_1 \in \mathbb{R}^n_1, \x_2 \in \mathbb{R}^n_2\}$, CCA learns the projections $W_1 \in \mathbb{R}^{n_1 \times m}$ and $W_2 \in \mathbb{R}^{n_2 \times m}$ which maximize the correlation between the projections $W_1^T\x_1$ and $W_2^T\x_2$.
% %
% The correlation between observations can thus be computed as the cosine distance between the mean-centered projections:
% %
% \begin{align}
% \text{corr}(\x_1, \x_2) = \frac{\phi(\x_1)^T\phi(\x_2)}{||\phi(\x_1)||_2||\phi(\x_2)||_2},
% \end{align}
%
% with $\phi(\x_i) = W_i^T\x_i - \E_i[W_i^T\x_i]$.
% %
% We follow~\citet{Shi2019} by treating $\x_1$ and $\x_2$ as the ResNet-101 image features and a 300-d projection~\citet{bojanowski2016enriching} for the captions.
%
We report the correlations for cross generations in \cref{tab:corr} and also prove qualitative results in the Appendix\todo{update if space}.
%
Here we can see that \gls{MEME} consistently obtains higher correlations than MVAE across all supervision rates, and higher than MMVAE in the fully supervised case.
%
Generally, cross-generating images yields higher correlation values, possibly due to the difficulty in generating semantically meaningful text.
%
% We would like to highlight that typically, fully observing captions yields similar correlation values for Image $\rightarrow$ Caption and Caption $\rightarrow$ Image, which is not the case when fully observing images.
% %
% In this instance, the correlations when cross-generating a caption yields lower values---possibly due to the difficulty in generating semantically meaningful text.
We would like to highlight that typically fully observing images leads to poorer performance when cross-generating captions.
%
Again, possibly due to the difficulty in generating text, but also possibly due to a discord between how the latent space is structured, where a similar pattern emerged when MNIST was only partially observed.
%



\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Correlation Values for CUB cross generations. Higher is better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			& \multicolumn{5}{c}{Image $\rightarrow$ Captions}\\
			\cmidrule(r{12pt}){2-6}
			Model & GT & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ \\
			\midrule
			\gls{MEME}\textsubscript{Image} & {0.106 $\pm$ 0.000} & \textbf{0.064 $\pm$ 0.011} & \textbf{0.042 $\pm$ 0.005} & \textbf{0.026 $\pm$ 0.002} & \textbf{0.029 $\pm$ 0.003}\\
			MMVAE\textsubscript{Image} & 0.106 $\pm$ 0.000 & 0.060 $\pm$ 0.010 & - & - & - \\
			MVAE\textsubscript{Image} & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001 & -0.000 $\pm$ 0.004       &      0.001 $\pm$ 0.004        &      -0.001 $\pm$ 0.005 \\
			\cmidrule(r{12pt}){2-6}
			\gls{MEME}\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & \textbf{0.064 $\pm$ 0.011}  & \textbf{0.062 $\pm$ 0.006} & \textbf{0.048 $\pm$ 0.004} & \textbf{0.052 $\pm$ 0.002} \\
			MMVAE\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & 0.060 $\pm$ 0.010 & - & - & -  \\
			MVAE\textsubscript{Captions}  & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001       &       -0.000 $\pm$ 0.004       &      0.000 $\pm$ 0.003        &      0.001 $\pm$ 0.002   \\
			\cmidrule(r{12pt}){2-6}\\
			& \multicolumn{5}{c}{Caption $\rightarrow$ Image}\\
			\cmidrule(r{12pt}){2-6}
			Model & GT & $f = 1.0$ & $f = 0.5$ & $f = 0.25$ & $f = 0.125$ \\
			\midrule
			\gls{MEME}\textsubscript{Image} & 0.106 $\pm$ 0.000 & \textbf{0.074 $\pm$ 0.001} & \textbf{0.058 $\pm$ 0.002} &      \textbf{0.051 $\pm$ 0.001}  & \textbf{0.046 $\pm$ 0.004}  \\
			MMVAE\textsubscript{Image}  & 0.106 $\pm$ 0.000 & 0.058 $\pm$ 0.001 & - & - & -   \\
			MVAE\textsubscript{Image}  & 0.106 $\pm$ 0.000 & -0.002 $\pm$ 0.001 & -0.002 $\pm$ 0.000       &      -0.002 $\pm$ 0.001       &      -0.001 $\pm$ 0.001  \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{Captions} & 0.106 $\pm$ 0.000 & \textbf{0.074 $\pm$ 0.001} & 0\textbf{.059 $\pm$ 0.003} & \textbf{0.050 $\pm$ 0.001} & \textbf{0.053 $\pm$ 0.001}   \\
			MMVAE\textsubscript{Captions} & 0.106 $\pm$ 0.000 & 0.058 $\pm$ 0.001 & - & - & -  \\
			MVAE\textsubscript{Captions} & 0.106 $\pm$ 0.000 & 0.002 $\pm$ 0.001       &       -0.001 $\pm$ 0.002       &      -0.003 $\pm$ 0.002       &      -0.002 $\pm$ 0.001 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:corr}
\end{table}

\paragraph{Discussion} In this sub-section we outlined how \gls{MEME} is able to obtain good performance on cross-generation tasks when partially observing either modality.
%
One key result from theses experiments is the in-balance between results depending on which modality is observed, e.g. partially observing MNIST leads to poor cross-generations for MNIST $\rightarrow$ SVHN and partially observing captions leads to poor cross-generations for Image $\rightarrow$ Captions.
%
Hypothetically, this is not an unsurprising result, as the objective used here has been shown to structure the latent space~\citep{joy2021capturing} depending on the information from the other modalities, i.e. in their work they used labels enforce disentanglement of the latent factors.
%
Consequently, the structure of the latent space will change depending on which modality is partially observed, which in turn will have a subsequent knock-on effect on the generations.
%
%We further investigated this effect in \cref{app:results}, where we also present additional results on the performance of \gls{MEME}, but omitted them to the Appendix due to space constraints.
We will now investigate this phenomenon further by inspecting the structure of the latent representations.
%
We also present additional results on the performance of \gls{MEME}, but omitted them to the Appendix due to space constraints.

\subsection{Discriminative Task}\label{sec:disc}
%
We now investigate the structure of the learnt latent space.
%
One of the benefits from utilizing a VAE is the natural emergence of a representation, which can typically be used for interoperability or utilized in downstream tasks.
%
Here we again follow previous work~\citep{Shi2019, sutter2020multimodal, sutter2021generalized} by fitting a linear classifier to the latent space, allowing us to interpret the suitable for further downstream tasks.

Specifically, we learn a linear classifier on the latent space to predict the digit.
% 
A linear classifier which is able to obtain a high accuracy for classification indicates that the latent space is reasonably structured according to the underlying class.
%
We report the results in~\cref{tab:digit_acc}, where we see that our model is able to structure the latent space in such a way that digit classification can be extracted to a higher accuracy than for the other models.

Typically, given an SVHN image we obtain lower classification accuracies than if we were given an MNIST image.
%
We posit that this is due to the lack of structuring naturally occurring from SVHN.
%
We also see here that fully observing MNIST actually improves the classification score for SVHN (third row from bottom) than if we fully observe SVHN, this is due to the presence of MNIST causing the latent space to structure in a more suitable way for classification.

\paragraph{Discussion}
Here we see that the presence of MNIST improves performance on tasks centred on SVHN.
%
A similar effect was seen in the top row of~\cref{tab:coherence}, where fully observing SVHN led to unsuitable encodings to generate an SVHN image given a MNIST image, which could be correcting by fully observing MNIST instead.
%
The resulting conclusion is that the structuring of the latent representation for SVHN can adapt to that of SVHN, but not the other way around.
%
Consequently, when MNIST is present, it imposes a higher level of structure in the latent space, which is more suitable for tasks such as classification or cross-generation.


\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Latent Space Linear Digit Classification.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			& \multicolumn{5}{c}{MNIST}\\
			\cmidrule(r{12pt}){2-6}
			Model & $1.0$ & $0.5$ & $0.25$ & $0.125$ & $0.0625$ \\
			\midrule
			Ours\textsubscript{SVHN} & 0.903 $\pm$ 0.003 & 0.883 $\pm$ 0.003  & 0.874 $\pm$ 0.006 & 0.822 $\pm$ 0.003 & 0.796 $\pm$ 0.007 \\
			MMVAE\textsubscript{SVHN} & 0.886 $\pm$ 0.003  & - & - & - & - \\
			MVAE\textsubscript{SVHN} & 0.364 $\pm$ 0.0373  & 0.442 $\pm$ 0.123 & 0.526 $\pm$ 0.032  & 0.406 $\pm$ 0.132        & 0.438 $\pm$ 0.0826 \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{MNIST} & 0.903 $\pm$ 0.003 & 0.882 $\pm$ 0.003 & 0.844 $\pm$ 0.008 & 0.823 $\pm$ 0.002 & 0.806 $\pm$ 0.004 \\
			MMVAE\textsubscript{MNIST} & 0.886 $\pm$ 0.003  & - & - & - & -\\
			MVAE\textsubscript{MNIST}  & 0.364 $\pm$ 0.0373 & 0.452 $\pm$ 0.051  & 0.499 $\pm$ 0.078 & 0.566 $\pm$ 0.032 & 0.629 $\pm$ 0.006 \\    
			\cmidrule(r{12pt}){2-6}\\
			& \multicolumn{5}{c}{SVHN}\\
			\cmidrule(r{12pt}){2-6}
			Model & $1.0$ & $0.5$ & $0.25$ & $0.125$ & $0.0625$ \\
			\midrule
			Ours\textsubscript{SVHN} & 0.644 $\pm$ 0.007  & 0.540 $\pm$ 0.010 & 0.296 $\pm$ 0.022 & 0.143 $\pm$ 0.006 & 0.107 $\pm$ 0.005 \\
			MMVAE\textsubscript{SVHN} & 0.499 $\pm$ 0.045 & - & - & - & - \\
			MVAE\textsubscript{SVHN} & 0.12 $\pm$ 0.00569 & 0.111 $\pm$ 0.022        &      0.112 $\pm$ 0.001        &      0.105 $\pm$ 0.004        & 0.103 $\pm$ 0.004 \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{MNIST} & 0.644 $\pm$ 0.007  & 0.575 $\pm$ 0.011 & 0.394 $\pm$ 0.021 & 0.381 $\pm$ 0.008 & 0.369 $\pm$ 0.026 \\
			MMVAE\textsubscript{MNIST} & 0.499 $\pm$ 0.045 & - & - & - & -\\
			MVAE\textsubscript{MNIST} & 0.12 $\pm$ 0.00569  & 0.11 $\pm$ 0.00208 & 0.116 $\pm$ 0.0189 & 0.115 $\pm$ 0.0101 & 0.107 $\pm$ 0.00503  \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:digit_acc}
\end{table}

\subsection{Extracting Relatedness}\label{sec:relatedness}
%
When considering latent representations, we should be able to leverage them to obtain a sense of similarity between two inputs.
%
Providing that the latent space is structured in a sensible way, the distance between representations for two modalities should yield a strong indication of their similarity or relatedness.
%
One of the key advantages of our approach is that we see the structuring of the latent space become suitable for obtaining relatedness.
%
Moreover, a natural mechanism for extracting relatedness between samples naturally emerges that doesn't rely on the Euclidean distance between samples.

Because during training we regularize the encoding distributions to be near to each other when they are encoding a data-point with of a similar abstract concept, at test time we can compare the closeness of these distributions to extract a metric for relatedness.
%
Here we use the 2-Wasserstein distance --- a symmetric metric with closed form expression (see ~\cref{app:wassertein} for more details).
Specifically, we compute $d_{ij} = \calW_2(q(\z|\bs_i)||q(\z|\bt_j))$, where $q(\z|\bs_i)$ and $q(\z|\bt_j)$ are the individual encoders, for all combination of pairs $\{\bs_i, \bt_j\}$ in the mini-batch, i.e $\{\bs_i, \bt_j\} \in \mathcal{B}~\forall~i,~j\in\{1\dots ,M\}$ where $M$ is the number of elements in the mini-batch $\mathcal{B}$.
%
We then plot $d_{ij}$ on a histogram, and we color-code the histogram by whether the corresponding data pair $\{\bs_i, \bt_j\}$ are related.
%
Ideally, we should observe smaller distances between encoding distributions for data pairs that are related, and larger for the ones that are not.

% From this data, we can then construct two histograms which indicate the distribution of the distances for pairs which are matched and pairs which are not.
%
% Intuitively, a model which extracts relatedness successfully should have a higher mass for closer distances and lower mass for further distances when the samples \emph{are} related.
%
% The opposite is true for when they are not related, i.e. we should see a high mass at further distances.

See results in \cref{fig:histograms}.
%
We see that \gls{MEME} generally yields a higher mass at lower distance values for the matched case than it does for the unmatched case, indicating a high probability of closer distances when pairs are matched than when they are not.
%
MMVAE goes someway to obtaining a similar pattern, but falls short of achieving the same disparity as \gls{MEME}, the distributions for MVAE match completely, indicating a complete inability to extract relatedness.



\begin{figure}[h!]
	\centering
	\scalebox{0.9}{
	\begin{tabular}{ccc}
		\includegraphics[width=0.33\linewidth]{media/friday/ccvae_digits_histogram.png}&
		\includegraphics[width=0.33\linewidth]{media/friday/mmvae_digits_histogram.png}&			\includegraphics[width=0.33\linewidth]{media/friday/mvae_digits_histogram.png}	\\
		\includegraphics[width=0.33\linewidth]{media/friday/ccvae_cub_histogram.png}&
		\includegraphics[width=0.33\linewidth]{media/friday/mmvae_cub_histogram.png}&			\includegraphics[width=0.33\linewidth]{media/friday/mvae_cub_histogram.png}
	\end{tabular}
	}
	\caption{Histograms of Wassertein distance for SVHN and MNIST (Top) and CUB (Bottom): Ours (Left), MMVAE (middle) and MVAE (Right). Blue indicates unmatched samples and orange matched samples. We expect to see high densities of blue at further distances and visa-versa for orange.}
	\label{fig:histograms}
\end{figure}


\subsubsection{Multi-class distance Matrix}
%
For the MNIST-SVHN case, we can extract relatedness on a per-class basis.
%
Ideally, we want to see high relatedness when classes match and low relatedness when they do not.
%
To do this, we construct a distance matrix for the classes $\mathbf{K}\in\mathbb{R}^{10\times10}$, with each element corresponding to the average $\calW_2$ distance between encoding distributions of the corresponding classes.
%
I.e. for each batch, $K_{\{u, v\}} = \sum_{i\in\mathcal{I}}\sum_{j\in\mathcal{J}}d_{ij}~\text{s.t.}~\mathcal{I}=\{i \in \{1,\dots,M\}|\y_i = u\},~\mathcal{J}=\{j \in \{1,\dots,M\}|\y_j = v\}$, with $\y$ representing the class labels and then subsequently taking the average.
%
A perfect distance matrix will consist of a diagonal of all zeros and positive values in the off-diagonal.

We display the distance matrices, for the fully matched case in \cref{fig:confusion_mat}, where it can be seen that in general our method produces a lower diagonal, and a higher average distance for the off-diagonals.
%
MMVAE also obtains a lower diagonal, but also provides lower values for the off diagonals, MVAE is completely unable to extract relatedness.

Inspecting the confusion matrices further, we see some interesting features.
%
For instance, our model is able to extract the understanding that SVHN \texttt{3} is similar to MNIST \texttt{5} and \texttt{8} (fourth column), and that \texttt{1} and \texttt{0} are completely unrelated.
%
A similar pattern can be seen in MMVAE, but again this is not as pronounced and MVAE completely fails in this case.
%
To further extract this structure, we construct a dendrogram to visualize the hierarchical clustering of the relatedness, which we display in \cref{fig:confusion_mat}.
%
Again we see that our model is able to obtain a clustering which one would typically associate with a digit dataset.
%
E.g. \texttt{3}, \texttt{5} and \texttt{8} cluster together, along with \texttt{6} and then \texttt{9}, typically we see a clustering of digits which tend to have a smooth writing profile (e.g. \texttt{8}), before the clustering of digits with sharp angles, with \texttt{0} and \texttt{1} being the most different.
%
This is not the case for MMVAE, which seems to cluster in a different manner, and again MVAE completely fails.
%
It is also important to note the values at which the clustering occurs, a higher value indicated a much greater distance between clusters.
%
Generally the clusters obtained in \gls{MEME} are separated further apart than for MMVAE, indicated by higher values on the y axis of the dendrogram.


\begin{figure}[h!]
	\centering
	\scalebox{0.8}{
	\begin{tabular}{ccc}
		\includegraphics[width=0.3\linewidth]{media/friday/ccvae_confusion_mat.png}&
		\includegraphics[width=0.3\linewidth]{media/friday/mmvae_confusion_mat.png}&			\includegraphics[width=0.3\linewidth]{media/friday/mvae_confusion_mat.png}\\
		\includegraphics[width=0.3\linewidth]{media/friday/ccvae_dendrogram.png}&
		\includegraphics[width=0.3\linewidth]{media/friday/mmvae_dendrogram.png}&			\includegraphics[width=0.3\linewidth]{media/friday/mvae_dendrogram.png}
	\end{tabular}
	}
	\caption{Distance matrices for KL divergence between classes for SVHN and MNIST (Top) and dendrogram (Bottom) for: Ours (Left), MVAE (middle) and MMVAE (Right).}
	\label{fig:confusion_mat}

\end{figure}
%
To further quantify the relatedness numerically, we report the correlation coefficient for each distance matrix, as this gives us a notion of the relative distances between all classes.
%
Specifically, we treat the dimensions of the matrix as random variables and the entries as pseudo probabilities of relatedness.
%
This then allows us to compute the sample correlation coefficient between the modalities.
%
For further information please see \cref{app:corr_coef}.
%
We present these results in \cref{tab:cond_number}, where we see that we are consistently able to report high correlation values, indicating that our method is able to extract relatedness, even in that partially observed case.
%
\begin{table}[h]
	\centering
	\def\s{\hspace*{4ex}} \def\r{\hspace*{2ex}}
	\caption{Correlation Coefficient of Confusion Matrices. Higher is Better.}
	{\small
		\begin{tabular}{@{}r@{\s}c@{\r}c@{\r}c@{\r}c@{\r}c@{\s}}
			\toprule
			Model & $1.0$ & $0.5$ & $0.25$ & $0.125$ & $0.0625$ \\
			\midrule
			Ours\textsubscript{SVHN} & \textbf{0.493 $\pm$ 0.020}  & \textbf{0.238 $\pm$ 0.011} & \textbf{0.110 $\pm$ 0.005} & \textbf{0.055 $\pm$ 0.013} & \textbf{0.030 $\pm$ 0.009} \\
			MMVAE\textsubscript{SVHN} & 0.477 $\pm$ 0.013 & - & - & - & \\
			MVAE\textsubscript{SVHN} & -0.018 $\pm$ 0.021 & -0.005 $\pm$ 0.012 & 0.005 $\pm$ 0.060 & -0.002 $\pm$ 0.014  & 0.000 $\pm$ 0.002 \\
			\cmidrule(r{12pt}){2-6}
			Ours\textsubscript{MNIST} & \textbf{0.493 $\pm$ 0.020}  & \textbf{0.190 $\pm$ 0.012} & \textbf{0.084 $\pm$ 0.003} & \textbf{0.059 $\pm$ 0.005}  & \textbf{0.044 $\pm$ 0.003}  \\
			MMVAE\textsubscript{MNIST} & 0.477 $\pm$ 0.013 & - & - & - & - \\
			MVAE\textsubscript{MNIST} & -0.018 $\pm$ 0.021  & -0.002 $\pm$ 0.005 & 0.000 $\pm$ 0.001 & nan $\pm$ nan & nan $\pm$ nan \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:cond_number}
\end{table}


%\subsection{Complex Dataset}
%%
%We now turn out attention to the more complex dataset, CUB~\citet{WelinderEtal2010}, which consists of 11,788 photograph of birds in a variety of different natural scenes.
%%
%Each photograph is accompanied by 10 fine-grained captions, describing the features of the bird, (e.g. crown color, beak size, etc.), caption were generated by humans through Amazon Mechanical Turk.
%%
%An example image and caption is given in \cref{fig:cub_ex}.
%%
%Following~\citet{Shi2019}, we treat the image features as one modality and the captions as the other, avoiding blurry image generations~\citet{zhao2017towards}.
%%
%Features are extracted from an off-the-shelf pre-trained ResNet-101 network~\citet{resnet}.
%%
%To obtain a reconstructed image, we perform nearest neighbor lookup in the feature space using the reconstructed feature.
%%
%We utilize a CNN networks for text modality~\citet{kalchbrennerconvolutional, pham2016convolutional, massiceti2018}, and a Categorical distribution for the likelihood function.
%



% \begin{figure}
% 	\begin{tabular}{C{1.0cm}  L{11.5cm}}
% 		\includegraphics[width=\linewidth]{media/friday/cub/ccvae/image_7.png} &
% 		\texttt{<sos> this bird has a blue head and back, an orange breast, and cream wingbars lined with black coverts. <eos>}
% 	\end{tabular}
% 	\caption{Example CUB image and associated caption.}
% 	\label{fig:cub_ex}
% \end{figure}








%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/1.0/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $100\%$.}
%	\label{fig:embeddings_sup}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.5_a/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $50\%$ drop rate SVHN.}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.1_a/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $10\%$ drop rate SVHN.}
%\end{figure}
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.5_b/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $50\%$ drop rate MNIST.}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{tabular}{c}
%		\includegraphics[width=0.8\linewidth]{media/0.1_b/embedding.png}
%	\end{tabular}
%	\caption{TSNE plot (Left) and TSNE plot (Right) for $10\%$ drop rate MNIST.}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

